Conservative Q-Learning for Offline Reinforcement Learning

Effectively leveraging large, previously collected datasets in reinforcement learning (RL) is a key challenge for large-scale real-world applications. Offline RL algorithms promise to learn effective policies from previously-collected, static datasets without further interaction. However, in practice, offline RL presents a major challenge, and standard off-policy RL methods can fail due to overestimation of values induced by the distributional shift between the dataset and the learned policy, especially when training on complex and multi-modal data distributions. In this paper, we propose conservative Q-learning (CQL), which aims to address these limitations by learning a conservative Q-function such that the expected value of a policy under this Q-function lower-bounds its true value. We theoretically show that CQL produces a lower bound on the value of the current policy and that it can be incorporated into a policy learning procedure with theoretical improvement guarantees. In practice, CQL augments the standard Bellman error objective with a simple Q-value regularizer which is straightforward to implement on top of existing deep Q-learning and actor-critic implementations. On both discrete and continuous control domains, we show that CQL substantially outperforms existing offline RL methods, often learning policies that attain 2-5 times higher final return, especially when learning from complex and multi-modal data distributions.

==> exit__.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\@setckpt{NeuRIPS2019/defs}{
\setcounter{page}{1}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{NAT@ctr}{0}
\setcounter{Item}{0}
\setcounter{Hfootnote}{0}
\setcounter{bookmark@seq@number}{0}
\setcounter{parentequation}{0}
\setcounter{float@type}{8}
\setcounter{algorithm}{0}
\setcounter{ALC@unique}{0}
\setcounter{ALC@line}{0}
\setcounter{ALC@rem}{0}
\setcounter{ALC@depth}{0}
\setcounter{ContinuedFloat}{0}
\setcounter{subfigure}{0}
\setcounter{subtable}{0}
\setcounter{theorem}{0}
\setcounter{assumption}{0}
\setcounter{proposition}{0}
\setcounter{definition}{0}
\setcounter{corollary}{0}
\setcounter{lemma}{0}
\setcounter{definition1}{0}
}


==> experiments.tex <==
\section{Experimental Evaluation}
\label{sec:experiments}




We compare CQL to prior offline RL methods on a range of domains and dataset compositions, including continuous and discrete action spaces, state observations of varying dimensionality, and high-dimensional image inputs. We first evaluate actor-critic CQL, using CQL($\mathcal{H}$) from Algorithm~\ref{alg:practical_alg}, on continuous control datasets from the D4RL benchmark~\citep{d4rl}.
We compare to: prior offline RL methods that use a policy constraint -- BCQ~\citep{fujimoto2018off}, BEAR~\citep{kumar2019stabilizing} and BRAC~\citep{wu2019behavior}; standard SAC~\citep{haarnoja}, an off-policy actor-critic method that we adapt to offline setting; and a behavioral cloning (BC) baseline that imitates the data distribution. 

\begin{table*}[h]
\centering
\fontsize{8}{8}\selectfont

\begin{tabular}{l|r|r|r|r|r|r||r}
\hline
\textbf{Task Name} & \textbf{SAC} & \textbf{BC} & \textbf{BCQ} & \textbf{BEAR} & \textbf{BRAC-p} & \textbf{BRAC-v} & \textbf{CQL($\mathcal{H}$)}\\ \hline
halfcheetah-random &  2.1 & 30.5 & 2.2 & 25.5 & 23.5 & 28.1 & \textbf{35.4} \\
hopper-random & 9.8 & \textbf{11.3} & 9.2 & 9.5 & \textbf{11.1} & \textbf{12.0} & \textbf{10.8}\\
walker2d-random & 1.6 & 4.1 & 4.8 &  \textbf{6.7} & 0.8 & 0.5 & \textbf{7.0}\\ \hline
halfcheetah-medium & -4.3 & 36.1 & 35.4 & 38.6 & \textbf{44.0} & \textbf{45.5} & \textbf{44.4}\\
walker2d-medium & 0.9 & 6.6 & 19.2 & 33.2 & 72.7 & \textbf{81.3} & {79.2}\\
hopper-medium & 0.8 & 29.0 & 37.1 & 47.6 & 31.2 & 32.3 & \textbf{65.2}\\ \hline
halfcheetah-expert & -1.9 & \textbf{107.0} & \textbf{106.0} & \textbf{108.2} & 3.8 & -1.1 & {104.8}\\
hopper-expert & 0.7 & \textbf{109.0} & \textbf{107.6} & \textbf{110.3} & 6.6 & 3.7 & \textbf{109.9} \\
walker2d-expert & -0.3 & 125.7 & 128.5 & 106.1 & -0.2 & -0.0 & \textbf{153.9} \\ \hline
halfcheetah-medium-expert & 1.8 & 35.8 & 59.2 & 51.7 & 43.8 & 45.3 & \textbf{62.4}\\
walker2d-medium-expert & 1.9 & 11.3 & 19.1 & 10.8 & -0.3 & 0.9 & \textbf{98.7}\\
hopper-medium-expert & 1.6 & \textbf{111.9} & 66.6 & 4.0 & 1.1 & 0.8 & \textbf{111.0}\\ \hline
halfcheetah-random-expert & 53.0 & 1.3 & 59.6 & 24.6 & 30.2 & 2.2 & \textbf{92.5}\\
walker2d-random-expert & 0.8 & 0.7 & 0.0 & 1.9 & 0.2 & 2.7 & \textbf{91.1}\\
hopper-random-expert & 5.6 & 10.1 & 9.8 & 10.1 & 5.8 & 11.1 & \textbf{110.5} \\ \hline
halfcheetah-mixed & -2.4 & 38.4 & 29.5 & 36.2 & \textbf{45.6} & \textbf{45.9} & \textbf{46.2}\\
hopper-mixed & 3.5 & 11.8 & 15.7 & 25.3 & 0.7 & 0.8 & \textbf{70.3}\\
walker2d-mixed & 1.9 & 11.3 & 8.3 & 10.8 & -0.3 & 0.9 & \textbf{33.4}\\
\hline
\end{tabular}
\caption{\label{table:mujoco}{\small Performance of CQL($\mathcal{H}$) and prior methods on MuJoCo tasks from D4RL, on the normalized return metric. Note that CQL performs similarly or better than the best prior method with simple datasets, and greatly outperforms prior methods with complex distributions (``--mixed'', ``--random-expert'', ``--medium-expert'').}}
\normalsize
\vspace{-10pt}
\end{table*}


Results for the simpler gym domains are shown in Table~\ref{table:mujoco}. The results for BEAR, BRAC and BC are based on numbers reported by \citet{d4rl}. On the datasets generated from a single policy, marked as ``-random'', ``-expert'' and ``-medium'', CQL matches or exceeds the best prior methods, but by a small margin. However, on datasets that combine multiple policies (``-mixed'', ``-medium-expert'' and ``-random-expert''), that are more likely to be common in practical datasets, CQL outperforms prior methods by large margins, sometimes as much as \textbf{2-3x}.  




The more complex Adroit~\citep{rajeswaran2018dapg} tasks (Figure~\ref{fig:d4rl_tasks}) in D4RL require the agent to control a 24-DoF robotic hand, using limited data generated from real-world human demonstrations. These tasks are substantially more difficult than the gym tasks in terms of both the dataset composition and high-dimensionality. Prior offline RL methods generally struggle to learn meaningful behaviors on 
\begin{wrapfigure}{l}{0.55\textwidth}
  \vspace{-18pt}
  \begin{center}
    \includegraphics[width=0.2\textwidth]{images/antmaze_all.png}
    \includegraphics[width=0.16\textwidth]{images/adroit_all.png}
    \includegraphics[width=0.17\textwidth]{images/adept_franka_kitchen.png}
  \end{center}
  \vspace{-7pt}
  \caption{{\small Evaluation tasks in the D4RL suite (from L to R: AntMaze navigation, Adroit, Franka Kitchen tasks).}}
  \vspace{-14pt}
 \label{fig:d4rl_tasks}
\end{wrapfigure}
these tasks, and the strongest baseline is actually na\"{i}ve behavioral cloning. As shown in Table~\ref{table:adroit_antmaze}, CQL variants are the only methods that improves over na\"{i}ve behavioral
cloning, attaining scores that are \textbf{2-9x} those of the next best offline RL method. As discussed in Section~\ref{sec:framework}, CQL($\rho$), witrh $\rho = \policy^{k}$, i.e. the previous policy, outperforms CQL($\mathcal{H}$) on a number of these adroit tasks, due to the higher action dimensionality resulting in higher variance for the CQL($\mathcal{H}$) importance weights. However, both variants outperform prior methods.


The maze tasks in D4RL require composing pieces of suboptimal trajectories to form more optimal policies for traveling from a start state to a goal. 
While prior methods sometimes learn meaningful policies on the simpler U-maze, only CQL is able to make meaningful progress on the substantially harder medium and large mazes, achieving nearly \textbf{2-5x} higher return as compared to prior methods.

Finally, we evaluate CQL on the Franka kitchen domain~\citep{gupta2019relay} from D4RL~\citep{d4rl_repo}.
The goal is to control a 9-DoF robot in a kitchen environment. These tasks require manipulating multiple objects (microwave, kettle, etc.) sequentially in a single episode to reach a desired goal. The agent receives a sparse 0-1 completion reward. These tasks are especially challenging, since they require composing different parts of trajectories, precise long-horizon manipulation, and handling human-provided teleoperation data. As shown in Table~\ref{table:adroit_antmaze}, CQL outperforms prior methods in this setting, and is the only method that outperforms behavioral cloning, attaining over 40\% success rate on all tasks.



\begin{table}[]
\centering

\fontsize{8}{8}\selectfont

\begin{tabular}{l|l|r|r|r|r|r||r|r}
\hline
\textbf{Domain} & \textbf{Task Name} & \textbf{BC} & \textbf{SAC} & \textbf{BEAR} & \textbf{BRAC-p} & \textbf{BRAC-v} & \textbf{CQL($\mathcal{H}$)} & \textbf{CQL($\rho$)}\\ \hline
\multirow{6}*{AntMaze}
& antmaze-umaze & 65.0 & 0.0 & \textbf{73.0} & 50.0 & 70.0 & \textbf{74.0} & \textbf{73.5}\\
& antmaze-umaze-diverse  & 55.0 & 0.0 & 61.0 & 40.0 & 70.0 & \textbf{84.0} & 61.0\\
& antmaze-medium-play  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{61.2} & 4.6 \\
& antmaze-medium-diverse  & 0.0 & 0.0 & 8.0 & 0.0 & 0.0 & \textbf{53.7} & 5.1 \\
& antmaze-large-play & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{15.8} &  3.2\\
& antmaze-large-diverse & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{14.9} & 2.3 \\
\hline
\multirow{8}*{Adroit}
& pen-human  & 34.4 & 6.3 & -1.0 & 8.1 & 0.6 & 37.5 & \textbf{55.8}\\
& hammer-human & 1.5 & 0.5 & 0.3 & 0.3 & 0.2 & \textbf{4.4} & {2.1}\\
& door-human & 0.5 & 3.9 & -0.3 & -0.3 & -0.3 & \textbf{9.9} & \textbf{9.1} \\
& relocate-human & 0.0 & 0.0 & -0.3 & -0.3 & -0.3 & 0.20 & \textbf{0.35}\\
& pen-cloned  & \textbf{56.9} & 23.5 & 26.5 & 1.6 & -2.5 & 39.2 & 40.3\\
& hammer-cloned & 0.8 & 0.2 & 0.3 & 0.3 & 0.3 & 2.1 & \textbf{5.7} \\
& door-cloned & -0.1 & 0.0 & -0.1 & -0.1 & -0.1 & 0.4 & \textbf{3.5}\\
& relocate-cloned & \textbf{-0.1} & -0.2 & -0.3 & -0.3 & -0.3 & \textbf{-0.1} & \textbf{-0.1}\\
\hline
\multirow{3}*{Kitchen}
& kitchen-complete & 33.8 & 15.0 & 0.0 & 0.0 & 0.0 & \textbf{43.8} & 31.3\\
& kitchen-partial & 33.8 & 0.0 & 13.1 & 0.0 & 0.0 & \textbf{49.8} & \textbf{50.1} \\
& kitchen-undirected & 47.5 & 2.5 & 47.2 & 0.0 & 0.0 & \textbf{51.0} & \textbf{52.4} \\ \hline
\end{tabular}
\normalsize
\caption{\label{table:adroit_antmaze}{\small Normalized scores of all methods on AntMaze, Adroit, and kitchen domains from D4RL, averaged across 4 seeds. On the harder mazes, CQL is the \textit{only} method that attains non-zero returns, and is the only method to outperform simple behavioral cloning on Adroit tasks with human demonstrations.
The CQL($\rho$) variant, which avoids importance weights, is more stable on the higher-dimensional Adroit tasks.}}
\vspace{-25pt}
\end{table}


Lastly, we evaluate a discrete-action Q-learning variant of CQL (Algorithm~\ref{alg:practical_alg}) on image-based Atari games~\citep{bellemare2013arcade}. We compare CQL to REM~\citep{agarwal2019optimistic} and QR-DQN~\citep{dabney2018distributional} on the four Atari tasks that are evaluated in detail by \citet{agarwal2019optimistic}, using the dataset released by the authors: Pong, Breakout, Qbert and Seaquest. We were not able to reproduce the QR-DQN and REM results on Asterix using the official implementation and data from \citet{agarwal2019optimistic}, and no method was able to perform well on the provided data for this task, but we include the scores in Table~\ref{table:atari_reduced_size}.
\begin{figure*}[h]
\vspace{-10pt}
  \includegraphics[width=0.23\linewidth]{images/pong.pdf}  
  \includegraphics[width=.23\linewidth]{images/breakout.pdf}  
  \includegraphics[width=.23\linewidth]{images/qbert.pdf}  
  \includegraphics[width=.23\linewidth]{images/seaquest.pdf}  
\caption{\label{fig:cql_20m_atari}{\footnotesize Performance of CQL, QR-DQN and REM as a function of training steps (x-axis) in setting \textbf{(2)} when provided with only the first 20\% of the samples of an online DQN run. Note that CQL is able to learn stably on 3 out of 4 games, and its performance does not degrade as steeply as QR-DQN on Seaquest.}}
\vspace{-10pt}
\end{figure*}
Following the evaluation protocol of \citet{agarwal2019optimistic}, we evaluated on two types of datasets, both of which were generated from the DQN-replay dataset:
\textbf{(1)} a dataset consisting of the first 20\% of the samples observed by an online DQN agent (Fig. 7 in \citep{agarwal2019optimistic}) and 
\textbf{(2)} datasets consisting of only 1\%  and 10\% of the samples in the replay buffer of an online DQN agent (Fig. 6 in \citep{agarwal2019optimistic}). In setting \textbf{(1)}, shown in Figure~\ref{fig:cql_20m_atari}, CQL generally achieves similar or better performance over the course of training as QR-DQN and REM.
When only using only 1\% or 10\% of the data, in setting \textbf{(2)}, we see in Table~\ref{table:atari_reduced_size} that CQL substantially outperforms REM and QR-DQN, especially in the harder 1\% condition, where performance exceeds the best prior method by as much as \textbf{28x} on Q*bert, and \textbf{6x} on Breakout.

\begin{table}[h]
    \centering
    \begin{tabular}{l|r|r|r|||r|r|r}
    \hline
        \textbf{Task Name} & \textbf{QR-DQN} & \textbf{REM} & \textbf{CQL($\mathcal{H}$)}  & \textbf{QR-DQN} & \textbf{REM} & \textbf{CQL($\mathcal{H}$)}  \\
        \hline
         Pong & 3.0 & 6.0 & \textbf{19.3} & 16.7 & 16.8 & \textbf{18.5} \\
         Breakout & 7.8 & 9.2 & \textbf{61.1} & 176.0 & 96.0 & \textbf{269.3} \\
         Q*bert & 500.0 & 500.0 & \textbf{14012.0}& 11201.8 & 8070.2 & \textbf{13855.6}\\
         Seaquest & 480.2 & 390.1 & \textbf{779.4} & 3300.0 & \textbf{4290.4} & 3674.1 \\
         Asterix\footnote{No method (CQL or prior methods, REM and QR-DQN, were able to attain non-trivial performance on this game using the dataset provided by \citet{agarwal2019optimistic}} & 166.3 & 386.5 & \textbf{592.4} & 189.2 & 75.1 & 156.3 \\
         \hline
    \end{tabular}
    \caption{{\footnotesize CQL, REM and QR-DQN in setting \textbf{(1)} with 1\% data (left), and 10\% data (right). CQL drastically outperforms prior methods with 1\% data, and usually attains better performance with 10\%.}}
    \label{table:atari_reduced_size}
\end{table}






==> method.tex <==
\vspace{-5pt}
\section{The Conservative Q-Learning (CQL) Framework}
\vspace{-5pt}
In this section, we develop a conservative Q-learning (CQL) algorithm, such that the expected value of a policy under the learned Q-function lower-bounds its true value. A lower bound on the Q-value prevents the over-estimation that typically appear in in offline RL settings due to OOD actions, access to only limited samples, uncertainty, and function approximation error~\citep{levine2020offline,kumar2019stabilizing}. 
We start by focusing on the policy evaluation step in CQL, which can be used by itself as an off-policy evaluation procedure, or integrated into a complete offline RL algorithm, as we will discuss in Section~\ref{sec:framework}.

\subsection{Conservative Off-Policy Evaluation (OPE)}
\label{sec:policy_eval}
\vspace{-5pt}
We aim to estimate the value, $V^\policy(\bs)$ of a target policy $\policy$ given access to a dataset, $\mathcal{D}$, generated by following a behavior policy $\behavior(\ba|\bs)$.
Because we are interested in preventing overestimation of the policy value, we learn a \textit{conservative}, lower-bound Q-function by additionally minimizing Q-values alongside a standard Bellman error objective. 

A natural choice of penalty is to minimize the expected Q-value under a particular distribution, $\mu(\bs, \ba)$. Since standard Q-function training does not query the Q-function value at unobserved states, but queries the Q-function at unseen actions, 
we restrict $\mu$ to match the state-marginal in the dataset,
such that $\mu(\bs, \ba) = d^\behavior(\bs) \mu(\ba|\bs)$, and only vary the conditional action distribution\footnote{In Appendix~\ref{app:error_bound_analysis}, we discuss how the policy value can be computed without querying the Q-function at a variable state distribution, justifying the sufficiency of this particular choice of $\mu(\bs, \ba)$.}.
This gives rise to the following objective for training the Q-function, as a function of a tradeoff factor $\alpha$:
\begin{equation}
    \small{\hat{Q}^{k+1} \leftarrow \arg\min_{Q}~ \alpha~ \E_{\bs \sim d^\behavior(\bs), \ba \sim \mu(\ba|\bs)}\left[Q(\bs, \ba)\right] + \frac{1}{2}~ \E_{\bs, \ba \sim d^\behavior(\bs) \behavior(\ba|\bs)}\left[\left(Q(\bs, \ba) - \bellman^\policy \hat{Q}^{k} (\bs, \ba) \right)^2 \right],} 
    \label{eqn:objective_1}
\end{equation}
In Proposition~\ref{thm:min_q_underestimates}, we will show that the resulting Q-value iterates, $\hat{Q}^k$, lower-bound the true Q-value iterate, $Q^k$, obtained by performing each iteration of exact policy evaluation, in the absence of function approximation (i.e., in the tabular setting).
As a consequence, the Q-values $\hat{Q}^\policy$ estimated by this procedure lower bound the actual Q-function of the policy, $Q^\policy$. 

While the penalty in Equation~\ref{eqn:objective_1} yields lower-bound estimates of the actual Q-function iterate, thus  
$\E_{\pi}[\hat{Q}(\bs, \ba)] \leq \E_{\pi}[Q(\bs, \ba) ] = V^\pi(\bs)$, 
this bound can be substantially tightened. Equation~\ref{eqn:objective_1} results in uniform underestimates of the value for any state.
Fortunately, since we are \textit{only} interested in estimating the value of the policy $\policy(\ba|\bs)$, we can obtain a much tighter conservative Q-function by instead only requiring the expected value of the Q-function under $\policy(\ba|\bs)$ to lower-bound its true expected value. We can obtain such an estimate by introducing an additional Q-value \textit{maximization} term under the data distribution, $\behavior(\ba|\bs)$, resulting in the objective (changes from Equation~\ref{eqn:objective_1} in red):
\begin{multline}
    \small{\hat{Q}^{k+1} \leftarrow \arg\min_{Q}~~ \alpha \cdot \left(\E_{\bs \sim d^\behavior(\bs), \ba \sim \mu(\ba|\bs)}\left[Q(\bs, \ba)\right] - \textcolor{red}{\E_{\bs \sim d^\behavior(\bs), \ba \sim \behavior(\ba|\bs)}\left[Q(\bs, \ba)\right]} \right)} \\
    \small{+ \frac{1}{2}~ \E_{\bs, \ba, \bs' \sim \mathcal{D}}\left[\left(Q(\bs, \ba) - \bellman^\policy \hat{Q}^{k} (\bs, \ba) \right)^2 \right]}.
    \label{eqn:modified_policy_eval}
\end{multline}
In Theorem~\ref{thm:cql_underestimates}, we show that the resulting Q-value, 
$\hat{Q}^{\policy}$ may not lower-bound ${Q}^\policy$ at each state-action pair, but the expected Q-value under $\policy$, $\E_{\policy(\ba|\bs)}[Q(\bs, \ba)]$,
is always lower-bounded, when $\mu(\ba|\bs) = \policy(\ba|\bs)$. Intuitively, since Equation~\ref{eqn:modified_policy_eval} maximizes Q-values under the dataset action distribution $\behavior$, Q-values for actions with higher density under $\behavior$ might overestimated, and thus the resulting value estimate is \textit{strictly} less conservative as compared to the point-wise lower bound estimate obtained via Equation~\ref{eqn:objective_1}. We also remark that, while in principle, the maximization term can utilize other distributions, besides the behavior policy $\behavior(\ba|\bs)$, however, we prove in Appendix~\ref{app:maximizing_distributions} that the resulting value estimate need not be a lower bound, if any other distribution besides $\behavior(\ba|\bs)$ is used.


\textbf{Theoretical analysis.} We now present the lower-bound results discussed above. For clarity, our results below do not consider potential over-estimatation that occurs as a result of access to only limited number of samples $\mathcal{D}$, or due to stochastic optimization, but we show how to incorporate such terms into all of our analysis in Appendix~\ref{app:handling_unobserved_actions}. Here, we first show that the Q-function learned by optimizing Equation~\ref{eqn:objective_1} lower-bounds the true Q-function. All proofs can be found in Appendix~\ref{app:missing_proofs}.
\begin{proposition}[Equation~\ref{eqn:objective_1} results in a lower bound]
\label{thm:min_q_underestimates}
For any $k \in \mathbb{N}$ and any $\mu(\ba|\bs)$, the Q-function iterate obtained from Equation~\ref{eqn:objective_1}, $\hat{Q}^k$, lower-bounds the actual Q-function iterate, $Q^k$, obtained by running exact policy evaluation.
That is, $\hat{Q}^k(\bs, \ba) \leq Q^k(\bs, \ba), \forall \bs, \ba$. 
The resulting asymptotic ($k \rightarrow \infty$) estimate of the policy value satisfies: 
\begin{equation*}
\forall \bs, \ba, ~~ \hat{Q}^\policy(s, a) = Q^\policy(\bs, \ba) - \left(I - \gamma P^\pi \right)^{-1} \left[\frac{\mu(\ba|\bs)}{\behavior(\ba|\bs)} \right](\bs, \ba) \leq Q^\policy(\bs, \ba).    
\end{equation*}
\end{proposition}

Next, we show that Equation~\ref{eqn:modified_policy_eval} lower-bounds the expected value under the policy $\policy$, when $\mu = \policy$. We further show that Equation~\ref{eqn:modified_policy_eval} does not lower-bound the Q-value estimates pointwise.
\begin{theorem}[Equation~\ref{eqn:modified_policy_eval} results in a tighter lower bound]
\label{thm:cql_underestimates}
For any $k \in \mathbb{N}$, the value of the policy under the Q-function iterate from Equation~\ref{eqn:modified_policy_eval}, $\hat{V}^k = \E_{\policy(\ba|\bs)}[\hat{Q}^k(\bs, \ba)]$, lower-bounds the true value of the policy obtained via exact policy evaluation, $V^k = \E_{\policy(\ba|\bs)}[Q^k(\bs, \ba)]$ when $\mu = \policy$, 
and the resulting asymptotic ($k \rightarrow \infty$) estimate of the policy value satisfies: 
\begin{equation*}
\forall \bs, ~~ \hat{V}^\policy(\bs) = V^\policy(\bs) - \left(I - \gamma P^\pi \right)^{-1} \E_{\policy(\ba|\bs)}\left[\frac{\policy(\ba|\bs)}{\behavior(\ba|\bs)} - 1 \right](\bs) \leq V^\policy(\bs).    
\end{equation*}
\end{theorem}


The analysis presented above assumes that no function approximation is used in the Q-function, meaning that each iterate can be represented exactly.
In Theorem~\ref{thm:policy_eval_func_approx}, we generalize this analysis to linear function approximation, where the amount of underestimation is state-dependent.
\begin{theorem}
\label{thm:policy_eval_func_approx}
Assume that the Q-function is represented as a linear function of given state-action feature vectors $\Qfeat$, i.e., $Q(s, a) = w^T \Qfeat(s, a)$. Let $D = \text{diag}\left(d^\behavior(\bs) \behavior(\ba|\bs)\right)$ denote the diagonal matrix with data density, and assume that $\Qfeat^T D \Qfeat$ is invertible. Then, the expected value of the policy under Q-value from Eqn~\ref{eqn:modified_policy_eval} at iteration $k+1$, $\E_{d^\behavior(\ba)}[\hat{V}^{k+1}(\bs)] = \E_{d^\behavior(\bs), \policy(\ba|\bs)}[\hat{Q}^{k+1}(\bs, \ba)]$, lower-bounds the corresponding tabular value, $\E_{d^\behavior(\bs)}[V^{k+1}(\bs)] =\E_{d^\behavior(\bs), \policy(\ba|\bs)}[Q^{k+1}(\bs, \ba)]$, if
\begin{equation*}
\small{\alpha_k \geq \max \left(\frac{D^T\left[\Qfeat \left(\Qfeat^T D \Qfeat \right)^{-1} \Qfeat^T - I \right]\left((\bellman^\policy \hat{Q}^k)(\bs, \ba)\right)}{D^T\left[ \Qfeat \left(\Qfeat^T D \Qfeat \right)^{-1} \Qfeat^T \right] \left(D \left[\frac{\policy(\ba|\bs) - \behavior(\ba|\bs)}{\behavior(\ba|\bs)} \right] \right)},~ 0 \right).}
\end{equation*}
\end{theorem}
The choice of $\alpha_k$ in Theorem~\ref{thm:policy_eval_func_approx} intuitively amounts to compensating for overestimation in value induced if the true value function cannot be represented in the chosen linear function class (numerator), by the potential decrease in value due to the CQL regularizer (denominator). This implies that if the actual value function can be represented in the linear function class, such that the numerator can be made $0$, then any $\alpha > 0$ is sufficient to obtain a lower bound. We prove this result in Appendix~\ref{app:missing_proofs}. 

We can generalize Theorem~\ref{thm:policy_eval_func_approx} to non-linear function approximation, such as neural networks, assuming that each iteration $k$ is performed by a single step of gradient descent on Equation~\ref{eqn:modified_policy_eval}, rather than a complete minimization of this objective. As we show in Corollary~\ref{corr:nonlinear_ntk}, by choosing $\alpha_k$ suitably, CQL learns provably lower-bounded values. We will also empirically show in Appendix~\ref{app:additional_results} that CQL can learn effective conservative Q-functions with multilayer neural networks.


\vspace{-5pt}
\subsection{Conservative Q-Learning for Offline RL}
\label{sec:framework}

We now build on the ideas in Section~\ref{sec:policy_eval}
to develop a general approach for offline policy learning, which we refer to as conservative Q-learning (CQL). 
As discussed in Section~\ref{sec:policy_eval}, we can obtain Q-value estimates such that value of a policy $\policy$
is lower-bounded by solving Equation~\ref{eqn:modified_policy_eval} with $\mu = \policy$. How should we utilize this for policy optimization? In principle, we could alternate between performing full off-policy evaluation for each policy iterate, and one step of policy improvement. However, this can be computationally expensive and may limit the algorithm performance due to Q-function overfitting~\citep{fu2019diagnosing}. Alternatively, since the policy $\policy$ is typically derived from the Q-function, either via greedy maximization, 
or via soft maximization, we could instead choose $\mu(\ba|\bs)$ to approximate the policy that would maximize the current Q-values, giving rise to an online algorithm.

We can formally capture this intuition by defining a family of optimization problems over the variable $\mu(\ba|\bs)$.
This family of optimization problems, with modifications from Equation~\ref{eqn:modified_policy_eval} marked in red, is shown in Equation~\ref{eqn:cql_framework}. An instance of this family is denoted by CQL($\mathcal{R}$) and is characterized by a particular choice of concave regularizer $\mathcal{R}(\mu)$:
\begin{multline}
    \label{eqn:cql_framework}
    \small{\min_{Q} \textcolor{red}{\max_{\mu}}~~ \alpha \left(\E_{\bs \sim d^\behavior(\bs), \ba \sim \textcolor{red}{\mu(\ba|\bs)}}\left[Q(\bs, \ba)\right] - \E_{\bs \sim d^\behavior(\bs), \ba \sim \behavior(\ba|\bs)}\left[Q(\bs, \ba)\right] \right)}\\
    \small{+ \frac{1}{2}~ \E_{\bs, \ba, \bs' \sim \mathcal{D}}\left[\left(Q(\bs, \ba) - \bellman^{\policy_k} \hat{Q}^{k} (\bs, \ba) \right)^2 \right] + \textcolor{red}{\mathcal{R}(\mu)} ~~~ \left(\text{CQL}(\mathcal{R})\right).}
\end{multline}

\textbf{Variants of CQL.} To demonstrate the generality of the CQL family of optimization problems, we discuss two specific instances within this family that are of special interest, and we evaluate them empirically in Section~\ref{sec:experiments}. First, if we choose $\mathcal{R}(\mu) = 0$, we obtain \mbox{$\mu(\ba|\bs) = \delta(\ba = \arg\max_{a} {Q}(\bs, \ba))$}, which is the ``greedy" distribution (analogous to a greedy policy) corresponding to $Q$. Second, if we choose $\mathcal{R}(\mu)$ to be the KL-divergence against a prior distribution, $\rho(\ba|\bs)$, i.e., $\mathcal{R}(\mu) = D_{\mathrm{KL}}(\mu, \rho)$, then we obtain $\mu(\ba|\bs) \propto \rho(\ba|\bs) \cdot \exp (Q(\bs, \ba))$ (for a derivation, see Appendix~\ref{app:cql_variants}). If $\rho = \text{Unif}(\ba)$,
then the first term in Equation~\ref{eqn:cql_framework} corresponds to a soft-maximum of the Q-values at any state $\bs$ and gives rise to the following variant of Equation~\ref{eqn:cql_framework}, referred as CQL($\mathcal{H}$):
\begin{equation}
    \small{\min_{Q}~ \alpha \E_{\bs \sim d^\behavior(\bs)}\left[\log \sum_{\ba} \exp(Q(\bs, \ba))\!-\!\E_{\ba \sim \behavior(\ba|\bs)}\left[Q(\bs, \ba)\right]\right]\!+\!\frac{1}{2}\!\E_{\bs, \ba, \bs' \sim \mathcal{D}}\left[\left(Q - \bellman^{\policy_k} \hat{Q}^{k} \right)^2 \right]\!.}
    \label{eqn:practical_objective}
\end{equation}
On the other hand, if $\rho(\ba|\bs)$ is chosen to be the behavior policy $\behavior$ or the previous policy $\policy^{k-1}$, the first term in Equation~\ref{eqn:practical_objective} is replaced by an exponential weighted average of Q-values of actions drawn from the chosen $\rho(\ba|\bs)$. Empirically, we find that this variant can be more stable on tasks with high-dimensional action spaces (e.g., Table~\ref{table:adroit_antmaze}) where it is challenging to estimate $\log \sum_{\ba} \exp$ via sampling due to high variance. In Appendix~\ref{app:cql_variants}, we discuss additional variants of CQL, which can be derived via a connection to distributionally robust optimization~\citep{namkoong2017variance}.  

We will discuss a practical instantiation of a deep RL algorithm based on CQL in Section~\ref{sec:practical_alg}. More generally, CQL can be instantiated as either a Q-learning algorithm (with $\bellman^*$ instead of $\bellman^{\policy}$ in Equations~\ref{eqn:cql_framework}, \ref{eqn:practical_objective}) or as an actor-critic algorithm. When Q-learning is used, exact maximization or an approximate maximization scheme, such as CEM~\citep{kalashnikov2018qtopt}, may be used to recover the greedy policy. In an actor-critic algorithm, a separate policy is trained to maximize the Q-value (Section~\ref{sec:background}).

\textbf{Theoretical analysis of CQL.}
Next, we will theoretically analyze CQL to show that the policy updates derived in this way are indeed ``conservative'', in the sense that each successive policy iterate is optimized against a lower bound on its value. Theorem~\ref{thm:cql_underestimation} shows that any instance of the CQL family learns Q-value estimates that lower-bound the actual Q-function under the action-distribution defined by the policy, $\policy^{k}$, under mild regularity conditions (slow updates to the policy).
\begin{theorem}[CQL learns lower-bounded Q-values]
\label{thm:cql_underestimation}
Assume that $D_{\mathrm{TV}}(\policy^{k+1}, \exp(\hat{Q}^k)) \leq \varepsilon$ (i.e., $\policy^k$ changes slowly w.r.t to $Q^k$). Then, the expected Q-value, $\hat{Q}^k$, lower-bounds the expected actual policy Q-value, that is, $\hat{V}^k(\bs) = \E_{ \policy^{k+1}(\ba|\bs)}[\hat{Q}^{k+1}(\bs, \ba)] \leq \E_{\policy^{k+1}(\ba|\bs)}[Q^{k+1}(\bs, \ba)] = V^k(\bs)$ if
\begin{equation*}
\small{\sum_{\ba} \exp(\hat{Q}^k(\bs, \ba)) \left[ \frac{\exp(\hat{Q}^k(\bs, \ba))}{\behavior(\ba|\bs)} -1 \right] \geq \max_{\ba \text{~s.t.~} \behavior(\ba|\bs) > 0} \left(\frac{\exp(\hat{Q}^k(\bs, \ba))}{\behavior(\ba|\bs)} \right) \cdot \varepsilon}. 
\end{equation*}
\end{theorem}
The LHS of the inequality above is equal to amount of underestimation caused in the value, $\hat{V}^{k+1}(s)$ if we the learned policy was equal to soft-optimal policy, $\exp(\hat{Q}^k)$, corresponding to the current Q-function, however, since the actual policy in an actor critic algorithm, $\policy^{k+1}$ may be different from this Boltzmann distribution, the amount of potential overestimation caused due to this difference is shown in the RHS. In order to obtain a lower bound, the amount of underestimation should be higher.  

Our next result shows that CQL Q-function update is ``gap-expanding,'' by which we informally mean that the difference in Q-values at in-distribution actions and over-optimistically erroneous out-of-distribution actions is higher than the corresponding difference under the actual Q-function. This is the reason why lower-bounded CQL values can especially help combat the detrimental effects of overestimation caused due to the distribution shift in the action distribution.
\begin{theorem}[CQL is gap-expanding] 
\label{thm:gap_amplify}
At any iteration $k$, CQL expands the difference in expected Q-values under the behavior policy $\behavior(\ba|\bs)$ and $\mu_k$, i.e., $\forall \bs, ~\E_{\behavior(\ba|\bs)}[\hat{Q}^k(\bs, \ba)] - \E_{\mu_k(\ba|\bs)}[\hat{Q}^k(\bs, \ba)] > \E_{\behavior(\ba|\bs)}[{Q}^k(\bs, \ba)] - \E_{\mu_k(\ba|\bs)}[{Q}^k(\bs, \ba)]$, for appropriate choices of $\alpha_k$.
\end{theorem}
We restate this theorem formally with a proof in Appendix~\ref{app:missing_proofs}. Theorem~\ref{thm:gap_amplify} shows that the suboptimality of the in-distribution actions ($\ba \sim \behavior$) under the learned Q-values is reduced. In scenarios where function approximation or stochastic approximation error makes OOD actions have higher learned Q-values, CQL backups that are more robust to Q-function estimation error by virtue of the gap-expanding property is appealing. 
As we will discuss in Section~\ref{sec:related} and Appendix~\ref{app:gap_amplify}, prior offline RL methods, that do not explicitly constrain or regularize the Q-function, may not enjoy such robustness properties, indicating the benefit of having a simple CQL regularizer. 

\vspace{-7pt}
\section{Practical Algorithm and Implementation Details}
\label{sec:practical_alg}
\vspace{-5pt}
We now describe two practical offline deep reinforcement learning methods based on CQL: a Q-learning variant and an actor-critic variant. Pseudocode is shown in Algorithm~\ref{alg:practical_alg}, with differences from conventional actor-critic algorithms (e.g., SAC~\citep{haarnoja}) and deep Q-learning algorithms (e.g., DQN~\citep{mnih2013playing}) in red.
Our algorithm uses the CQL($\mathcal{H}$) (or CQL($\mathcal{R}$) in general) objective from the CQL framework for training the Q-function $Q_\theta$, which is parameterized by a neural network with parameters $\theta$. For the actor-critic algorithm, a policy $\pi_\phi$ is trained as well. Our algorithm modifies the objective for the Q-function (swaps out Bellman error with CQL($\mathcal{H}$)) or CQL($\rho$)
\begin{wrapfigure}{r}{0.6\textwidth}
\begin{small}
\vspace{-23pt}
\begin{minipage}[t]{0.99\linewidth}
\begin{algorithm}[H]
\small
\caption{Conservative Q-Learning (both variants)}
\label{alg:practical_alg}
\begin{algorithmic}[1]
    \STATE Initialize Q-function, $Q_\theta$, and optionally a policy, $\pi_\phi$.
    \FOR{step $t$ in \{1, \dots, N\}}
        \STATE Train the Q-function using $G_Q$ gradient steps on objective from Equation~\ref{eqn:practical_objective} \\
        \mbox{$\theta_t := \theta_{t-1} - \eta_Q \nabla_\theta \textcolor{red}{\text{CQL}(\mathcal{R})(\theta)}$}\\
        (Use $\bellman^*$ for Q-learning, $\bellman^{\policy_{\phi_t}}$ for actor-critic)
        \STATE \underline{(only with actor-critic)} Improve policy $\pi_\phi$ via $G_\pi$ gradient steps on $\phi$ with SAC-style entropy regularization:\\
        \mbox{$\phi_{t} := \phi_{t-1} + \eta_\pi \mathbb{E}_{\bs \sim \mathcal{D}, \ba \sim \pi_\phi(\cdot|\bs)}[Q_\theta(\bs, \ba)\! -\! \log \pi_\phi(\ba|\bs)] $}
    \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-15pt}
\end{small}
\end{wrapfigure}
in a standard actor-critic or Q-learning setting, as shown in Line 3. As discussed in Section~\ref{sec:framework}, due to the explicit penalty on the Q-function, CQL methods do not require a policy constraint,
unlike prior offline RL methods~\citep{kumar2019stabilizing,wu2019behavior,siegel2020keep,levine2020offline}.
Hence, no fitting of a behavior policy $\behavior$ is required. This prevents the detrimental effects using an inaccurately fitted behavior policy in an offline RL algorithm~\citep{levine2020offline}.

\textbf{Implementation details.} Our algorithm requires an addition of only \textbf{20} lines of code on top of standard implementations of soft actor-critic (SAC)~\citep{haarnoja} for continuous control experiments and on top of QR-DQN~\citep{dabney2018distributional} for the discrete control experiments. The tradeoff factor, $\alpha$ is automatically tuned via Lagrangian dual gradient descent for continuous control, and is fixed at constant values described in Appendix~\ref{sec:experimental_details} for discrete control. We use default hyperparameters from SAC, except that the learning rate for the policy is chosen to be smaller. Elaborate details are provided in Appendix~\ref{sec:experimental_details}.  


==> old_theory.tex <==
\section{Why are Actor Constraints Insufficient with Function Approximation?}

Prior work has used actor constraints or penalties to prevent out-of-distribution action queries in the Q-function backup in the absence of function approximation. However, in this section, we demonstrate that actor constraints may be insufficient to provide effective learning progress in the presence of function approximation.
Our reasoning behind this statement is based on two reasons.
First, typical actor constraints or penalties aim at penalizing the learned actor, $\pi_\phi$ against
the effective Markovian policy for the dataset
defined as, $\pi_b(a|s) = \frac{\mu(s, a)}{\mu(s)}$. $\pi_b$ can be a highly multimodal and complex distribution, and the performance of most prior methods that rely on fitting an accurate parametric model for $\pi_b$, may thus be bottlenecked by the inability to fit this behavior distribution.

The second reason is more subtle. In scenarios where the dataset distribution, $\mu(s, a)$ is ``narrow'',
actor constraints or penalties may be insufficient to constrain the critic in the presence of function approximation, since the critic is trained by minimizing squared Bellman error on a narrow set of in-distribution actions (i.e., actions with $\mu(a|s) > 0$), and the Q-value outputs on other actions are pretty much uncontrolled.
Thus, generalization effects of the Q-function approximator may give rise erroneously over-optimistic Q-values on out-of-distribution actions, even when the target values are constrained to utilize in-distribution actions. When these erroneously high Q-values on out-of-distribution actions are then used to update the actor, it introduces errors in the actor, even in the presence of an actor penalty, which can slow down the amount of error accumulation in the actor, but not completely prevent it in certain scenarios.

In order to build intuition for the argument presented above, we will now present a simple didactic example of a 1D ``line-world'' MDP. This MDP has continuous states in the interval $[-1, 1]$ on the 1D number-line. At any state, there are two available actions: $a_1$, which transitions the agent to the left by $0.2$ units, and $a_2$ that transits the agent to the right by $0.2$ units.
The features provided for training a linear Q-function approximator are given by: $\phi(s, a_1) = s, \phi(s, a_2) = s + \varepsilon$, and the Q-function is parameterized via two scalar parameters, $w, b$. By suitably choosing the behavior policy density and the initialization of the Q-functions, for any given policy penalty coefficient, $\beta$,
we can set $\varepsilon$, such that a single gradient step on a uniform over actions initial policy, updates the actor towards choosing an out-of-distribution action $a$, for which $\pi_b(a|s) << 1$. 

The example provides some intuition for why actor penalties may not suffice when narrow distributions can induce erroneous critic generalization. In order to formally quantify the generalization effects induced in the Q-function, we assume that the Q-function is parameterized by $\theta \in \mathbb{R}^d$, and is updated via gradient descent, and 
compute the change in Q-values for a state action pair $(\bar{s}, \bar{a})$ due to a change in the parameter vector $\theta$ caused by the critic update, up to first order, as
\begin{equation}
\label{eqn:first_order}
    Q_{k+1}(\bar{s}, \bar{a}) \approx Q_{k}(\bar{s}, \bar{a}) - \alpha_k \expec_{s, a \sim \mu} [(Q_k(s, a) - \bellman^\pi \bar{Q}_k(s, a) ) \cdot k_\theta((s, a), (\bar{s}, \bar{a}))]
\end{equation}
where $k_\theta((s, a), (\bar{s}, \bar{a})) := \nabla_\theta Q_\theta(s, a)^T \nabla_\theta Q_\theta(\bar{s}, \bar{a})$ is the neural tangent kernel (NTK)~\citep{jacot18ntk}. 
When function approximation is not used, the corresponding Q-function iterate is given by:
\begin{equation}
\label{eqn:regular_update}
    Q_{k+1}(\bar{s}, \bar{a}) = Q_k(\bar{s}, \bar{a}) + \alpha_k \mu(\bar{s}, \bar{a}) (\bellman^\pi \bar{Q}_k(\bar{s}, \bar{a}) - Q_k(\bar{s}, \bar{a}))
\end{equation}
Now, we may ask: how does an update in Equation~\ref{eqn:first_order} affect the actor, which uses these new Q-values for its update? The policy update is:
\begin{equation}
\label{eqn:policy_constraint}
    \pi_{k+1} \leftarrow \max_{\pi}~~ \expec_{s \sim \mu(s)}\left[\expec_{a \sim \pi(\cdot|s)} [Q_{k+1}(s, a)] \right] + \beta D(\pi, \mu).
\end{equation}
Denoting $Q_{k+1}^{\text{no}}$ as the updated Q-function, $Q_{k+1}$, from Equation~\ref{eqn:regular_update}, and re-writing the policy update, we obtain:
\begin{equation}
    \pi_{k+1} \leftarrow \max_{\pi}~~~ \expec_{s \sim \mu(s)} \left[\expec_{a \sim \pi(\cdot|s)}[Q_{k+1}^{\text{no}}(s, a) + \alpha_k (K_\theta - I) \text{diag}(\mu) (\bellman^{\pi_k}\bar{Q}_k - Q_k)(s, a)] + \beta D(\pi, \mu) \right]
\end{equation}
Observe that the additional error in the Q-function due to function approximation can accidently lead to overestimated Q-values at out-of-distribution actions, as shown in the example discussed previously. Even when an actor penalty is used, as shown in Equation~\ref{eqn:policy_constraint}, the additional error in the Q-values can bias the policy towards actions that are sub-optimal. Note that this phenomenon is absent without function approximation, if Q-values at OOD actions are initialized to pessimistic values, since these are unaffected with the update shown in Equation~\ref{eqn:regular_update}. 

To summarize, the key issue here is the inability to control the function approximation error in the Q-function only via an actor constraint that can control target values, and the ability of this function approximation error to bias the policy towards OOD actions. As shown in our example, even in the presence of penalties on the actor, certain choices of features and initialization may prevent the actor from learning meaningfully, and enter into a cycle of gradual error accumulation. 
\textcolor{red}{AK: Probably add some stuff about how in an iterative sense this error accumulates. And put an example on a 1D lineworld, with linear function approximation that shows this issue. Or show a gridworld example.}


\section{Controlling Function Approximation Error via Penalized Q-Learning}

Now that we have seen that function approximation error in the Q-function -- which arises when backups are performed on certain choices of data distribution $\mu$ -- can cause problems with learning even in the presence of constrained bootstrapped target values, we seek a solution to this issue. A na\"ive solution would be to simply mimic tabular updates but with function approximators as previously explored in \citet{achiam2019towards}, however, this scheme is not desirable since computing gradient inner products ($K_\theta$) over all the states and empirically inverting the matrix $K_\theta$ is computationally extremely expensive. One can choose to just account for $K_\theta$ within a mini-batch, analogous to \citet{achiam2019towards}, however, this is not known to provide huge benefits and requires modifying substantial architectural details and design details for numerical stability reasons.

Instead, our approach, which we refer to as ALGONAME, chooses to penalize the Q-function under a suitably chosen ``negative'' distribution, and upweights Q-function values at in-distribution actions.
This ensures that the Bellman error minimization procedure does not erroneously downweight the Q-values at in-distribution actions and upweight those at out-of-distribution actions, as a consequence of function approximation. More concretely, our objective for training the Q-function, as shown in Equations~\ref{eqn:generic_new_update} and \ref{eqn:generic_new_update_2} now minimizes the Bellman error, subject to explicitly up-weighting Q-values on in-distribution actions while penalizing them on actions drawn from a different distribution $\nu$, which is of our choice. We refer to this family of optimization problems as: $\mathsf{PenalizedQ(\nu)}$. 
\begin{align}
    \label{eqn:generic_new_update}
    \mathsf{PenalizedQ(\nu)}:~~ \theta_{k+1} = \arg\min_{\theta} ~~& \sum_{i=1}^N \left( Q_\theta(s_i, a_i) - \bellman^\pi \bar{Q}(s_i, a_i) \right)^2 \\ %
    \text{s.t.}~~ & \expec_{s \sim \mu(s)}\left[ \expec_{a \sim \nu(\cdot|s)} [Q_\theta(s, a)] - \expec_{a \sim \mu(\cdot|s)}[Q_\theta(s, a)] \right] \leq \varepsilon
    \label{eqn:generic_new_update_2}
\end{align}
For different choices of the negative distribution $\nu$,
this objective amounts to solving different problems: If $\mu$
is chosen to be the Boltzmann distribution corresponding to the Q-function, i.e. $\nu(a|s) \propto \exp(Q_\theta(s, a))$, then, Equation~\ref{eqn:generic_new_update_2} is equivalent to penalizing the suboptimality of in-distribution actions,
$\mu(a|s)$ under the learned Q-function. If $\nu$ is chosen to be a function that is inversely proportional to the dataset action marginal, $\mu$, this amounts to penalizing the least likely actions in the dataset.

More generally, we can choose $\nu$ via a separate optimization procedure that optimizes $\mu$ subject to a concave regularizer $\mathcal{R}(\nu)$, giving rise to:
\begin{equation}
    \min_\theta~~ \max_\nu \sum_{i=1}^N \left( Q_\theta(s_i, a_i) - \bellman^\pi \bar{Q}\right)^2 + \beta \cdot \expec_{s \sim \mu}\left[ \expec_{a \sim \nu} [Q_\theta(s, a)] - \expec_{a \sim \mu}[Q_\theta(s, a)] \right] + \mathcal{R}(\nu)
\end{equation}
We provide two examples that are of special interest in our setting. When $\mathcal{R}(\nu)$ is chosen to be the Shannon entropy, $\mathcal{H}(\nu)$, we obtain the following objective:
\begin{equation}
\label{eqn:logsumexp_obj}
    \ell_{\mathcal{H}}(\theta) = \sum_{i=1}^N \left( Q_\theta(s_i, a_i) - \bellman^\pi \bar{Q}(s_i, a_i) \right)^2 + \beta \cdot \expec_{s \sim \mu}\left[\log \left( \int_{a} \exp(Q_\theta) \right) - \expec_{a' \sim \mu}[Q_\theta]\right]
\end{equation}
When $\mathcal{R}(\nu) = -\kldiv(\nu || \hat{\mu})$, where $\hat{\mu}$ denotes the empirical distribution of actions at a state, i.e. $\hat{\mu}(a_0|s_0) = \sum_{s_i, a_i \in \mathcal{D}} 1\{s_i = s_0, a_i = a_0 \} / \sum_{s_i} 1\{s_i = s_0\}$, then using the result from \citet{duchi2017variance}, we obtain the following variance-regularized objective:
\begin{equation}
\label{eqn:variance_regularized}
    \ell_{\mathcal{\kldiv(\hat{\mu})}}(\theta) = \sum_{i=1}^{|\mathcal{D}|} \left( Q_\theta(s_i, a_i) - \bellman^\pi \bar{Q}(s_i, a_i) \right)^2 + \beta \cdot \expec_{s \sim \mu} \sqrt{\frac{\var_{\hat{\mu}}\left( Q_\theta(s, \cdot) \right)}{|\mathcal{D}|}}
\end{equation}
We discuss several more objectives of the family arising from different choices of $\mathcal{R}$ in Appendix ??.

Next, we present our argument to show that our objective $\mathsf{Penalized}(\nu)$ solves the problem of incorrect generalization
in Q-functions, building on the argument from the previous section. As before, we compute an expression for Q-values after a gradient update.
For a particular state-action pair, $(\bar{s}, \bar{a})$, we can write:
\begin{equation}
\label{eqn:new_kernelized_update}
    Q_{k+1}(\bar{s}, \bar{a}) = Q_{k+1}^{\text{FQI}}(\bar{s}, \bar{a}) + \alpha_k \cdot \beta \cdot \expec_{s \sim \mu} [(\mu(a|s) - \nu(a|s)) \cdot k_\theta((s, a), (\bar{s}, \bar{a}))]
\end{equation}
We now provide an explanation centered around objective $\ell_\mathcal{H}(\theta)$ shown in Equation~\ref{eqn:logsumexp_obj}, but an explanation similarly follows for $\ell_{\mathcal{\kldiv(\hat{\mu})}}(\theta)$. If action $\bar{a}$ is out-of-distribution at state $\bar{s}$, an overestimation error that appears in $Q_{k+1}^{\text{FQI}}$ now gets nullified by an underestimation bias caused by $\mu(\bar{a}|\bar{s}) - \nu(\bar{a}|\bar{s})$, which will be a negative quantity if Q-value $Q_k(\bar{s}, \bar{a})$ is overestimated (since, $\nu(\bar{a}|\bar{s}) > \mu(\bar{a}|\bar{s})$). By suitably choosing weights $\beta$, we can ensure that Q-values are not high
for out-of-distribution actions. 


Finally, we present our practical actor-critic algorithm, ALGONAME, that uses Equation~\ref{eqn:logsumexp_obj} for learning effective policies for offline RL. Our algorithm is shown in Algorithm ??. It utilizes the framework of the soft-actor critic (SAC) algorithm, with the difference that the Q-function is trained via $\ell_\mathcal{H}(\theta)$ instead of simple Bellman error. The actor update is void of any special constraint, since the Q-function is trained to output smaller values for OOD actions.    


\subsection{Lower-Bound Argument}
While our motivation for optimization problems of the form of $\mathsf{Penalized}(\nu)$ was primarily based on considerations arising due to undesirable effects of function approximation,
in this section, we show that in settings without function approximation, ALGONAME that trains
Q-functions by optimizing $\ell_\mathcal{H}(\theta)$ and then using the corresponding Boltzmann policy for evaluation, gives rise to the strongest lower bound on the policy optimization objective.

First, note that the optimal solution to minimizing $\ell_\mathcal{H}$ at iteration $k$ of learning gives rise to the following Q-function iterate $Q_{k+1}$:
\begin{equation}
    \label{eqn:Q_iterate_tabular}
    Q_{k+1} = \bellman^{\pi_k} Q_{k} - \beta \cdot \left[\frac{\nu_k(a|s) - \mu(a|s)}{n(a|s)} \right]_{|S| \times |A|}
\end{equation}
where $n(a|s)$ denotes the number of times action $a$ is observed at state $s$ in dataset $\mathcal{D}$. Furthermore, note that $\nu_k(\cdot|s) = \pi_k(\cdot|s)$, since $\ell_{\mathcal{H}}$ is the chosen objective. Note also that the objective for training the actor via a gradient step
is given by $J_k(\pi) = \expec_{s \sim \mu(s)} \left[ \expec_{a \sim \pi_k(\cdot|s)}[Q_{k+1}(s, a) \right]$. By substituting Equation~\ref{eqn:Q_iterate_tabular} into this expression, we obtain
\begin{equation}
    J_k(\pi) = \expec_{s \sim \mu(s)} \left[ \expec_{a \sim \pi_k(\cdot|s)}[\bellman^{\pi_k} Q_k(s, a) - \beta (\pi_k(a|s) - \mu(a|s)) \right]
\end{equation}
Since the inner product of two vectors $\pi_k$, and $\mu$ cannot be more than the norm of $\pi_k$, we observe that $J_k(\pi) \leq \expec_{s \sim \mu(s)} \left[ \expec_{a \sim \pi_k(\cdot|s)}[\bellman^{\pi_k} Q_k(s, a)] \right] = \expec_{s \sim \mu(s)} \left[ \expec_{a \sim \pi_k(\cdot|s)}[Q_{k+1}(s, a)] \right]$, where the right hand side denotes the objective for policy improvement at iteration $k$ without any constraint. Note that this condition is strong, in that if $\nu_k(a|s) \neq \pi_k(a|s)$, then $J_k(\pi)$ may not be a lower bound for atleast one choice of the dataset distribution $\mu$.

Finally, we note that prior methods that penalize the target values instead incur an additional penalty due to the conservative estimates of target values used for backups. We discuss this in detail for two methods: BEAR and BRAC in Appendix ??.


